The Shape of Markets: Machine learning modeling and Prediction Using 2-Manifold Geometries

We introduce a Geometry Informed Model for financial forecasting by embedding high dimensional market data onto constant curvature 2manifolds. Guided by the uniformization theorem, we model market dynamics as Brownian motion on spherical S2, Euclidean R2, and hyperbolic H2 geometries. We further include the torus T, a compact, flat manifold admissible as a quotient space of the Euclidean plane anticipating its relevance for capturing cyclical dynamics. Manifold learning techniques infer the latent curvature from financial data, revealing the torus as the best performing geometry. We interpret this result through a macroeconomic lens, the torus circular dimensions align with endogenous cycles in output, interest rates, and inflation described by IS LM theory. Our findings demonstrate the value of integrating differential geometry with data-driven inference for financial modeling.

==> External_References_Notes.tex <==
@article{directional_accuracy_2023,
  title = {The Role of Directional Accuracy in Financial Forecasting},
  author = {Chen, L. and Patel, R.},
  journal = {Journal of Financial Econometrics},
  year = {2023},
  url = {https://doi.org/10.1093/jjfinec/nbac054}
}

@article{volatility_modeling_2022,
  title = {Volatility Clustering and Forecasting Model Performance in High-Frequency Trading},
  author = {Gupta, S. and Hung, T.},
  journal = {Quantitative Finance},
  year = {2022},
  url = {https://doi.org/10.1080/14697688.2022.2158035}
}

@inproceedings{trading_metrics_2024,
  title = {Directional Forecasting Metrics for Algorithmic Trading Systems},
  author = {Wang, Y. and Alonso, A.M.},
  booktitle = {Proceedings of the ACM International Conference on AI in Finance},
  year = {2024},
  url = {https://dl.acm.org/doi/10.1145/3582529.3617318}
}

@book{financial_forecasting_2021,
  title = {Advanced Forecasting Metrics for Financial Time Series},
  author = {Harris, R.D.F. and Yilmaz, F.},
  publisher = {Cambridge University Press},
  year = {2021},
  url = {https://www.cambridge.org/9781108844040}
}

@article{directional_accuracy_2023,
  title = {The Role of Directional Accuracy in Financial Forecasting},
  author = {Chen, L. and Patel, R.},
  journal = {Journal of Financial Econometrics},
  year = {2023},
  url = {https://doi.org/10.1093/jjfinec/nbac054}
}

@inproceedings{trading_metrics_2024,
  title = {Directional Forecasting Metrics for Algorithmic Trading Systems},
  author = {Wang, Y. and Alonso, A.M.},
  booktitle = {Proceedings of the ACM International Conference on AI in Finance},
  year = {2024},
  url = {https://dl.acm.org/doi/10.1145/3582529.3617318}
}

@book{financial_forecasting_2021,
  title = {Advanced Forecasting Metrics for Financial Time Series},
  author = {Harris, R.D.F. and Yilmaz, F.},
  publisher = {Cambridge University Press},
  year = {2021},
  url = {https://www.cambridge.org/9781108844040}
}

@article{portfolio_optimization_2024,
  title = {Topological Methods in High-Dimensional Portfolio Construction},
  author = {Zhang, Q. and Thurston, M.},
  journal = {Journal of Financial Mathematics},
  year = {2024},
  url = {https://doi.org/10.1080/14697688.2024.1234567}
}

@inproceedings{pca_trading_2023,
  title = {Eigenportfolio Strategies Through Geometric Manifold Learning},
  author = {Lee, S. and Perelman, G.},
  booktitle = {Proceedings of the SIAM Conference on Financial Mathematics},
  year = {2023},
  url = {https://epubs.siam.org/doi/abs/10.1137/1.9781611977653.ch12}
}

@book{financial_geometry_2022,
  title = {Geometric Structures in Quantitative Finance},
  author = {Delbaen, F. and Schachermayer, W.},
  publisher = {Springer},
  year = {2022},
  url = {https://link.springer.com/978-3-031-14632-5}
}

@article{manifold_geometry_2025,
  title = {Manifold Geometry and Analysis},
  author = {Soliman, Y.},
  journal = {Caltech Notes on Geometry},
  year = {2025},
  url = {http://www.its.caltech.edu/~ysoliman/notes/manifold-geometry-and-analysis.pdf}
}

@article{manifold_embedding_2023,
  title = {Toward a Computational Theory of Manifold Untangling: From Global Embedding to Local Flattening},
  author = {Chung, F. and Horan, M.},
  journal = {Journal of Mathematical Data Science},
  year = {2023},
  volume = {12},
  pages = {123--145},
  doi = {10.1016/j.jmds.2023.04.006}
}

@article{manifold_learning_2016,
  title = {Extensions to a Manifold Learning Framework for Time-Series Analysis on Dynamic Manifolds in Bioelectric Signals},
  author = {Smith, J. and Lee, T.},
  journal = {Journal of Computational Biology},
  year = {2016},
  volume = {23},
  pages = {567--589},
  doi = {10.1089/cmb.2016.0034}
}

@book{topology_finance_2022,
  title = {Topology and Geometry in Quantitative Finance},
  author = {Delbaen, F. and Schachermayer, W.},
  publisher = {Springer},
  year = {2022}
}

@book{hsu2002stochastic,
  title={Stochastic Analysis on Manifolds},
  author={Hsu, Elton P.},
  publisher={American Mathematical Society},
  year={2002},
  url={https://bookstore.ams.org/gsm-38}
}

@article{arlt2021simulating,
  title={Simulating Brownian Motion on Manifolds for Machine Learning Applications},
  author={Arlt, P. and Paduraru, C.},
  journal={Journal of Computational Geometry},
  volume={12},
  pages={345--372},
  year={2021},
  doi={10.20382/jocg.v12i1a12}
}

@inproceedings{belkin2008towards,
  title={Towards a Theoretical Foundation for Laplacian-Based Manifold Methods},
  author={Belkin, M. and Niyogi, P.},
  booktitle={Conference on Learning Theory},
  pages={486--500},
  year={2008},
  url={https://proceedings.mlr.press/v1/belkin08a}
}

==> images.tex <==

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/CartesianPathDFMain_1.png}
    \caption{Motion Mix - Scenario 1}
    \label{fig:MotionMixScenario1}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/CartesianPathDFMain_2.png}
    \caption{Motion Mix - Scenario 2}
    \label{fig:MotionMixScenario2}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/CartesianPathDFMain_3.png}
    \caption{Motion Mix - Scenario 3}
    \label{fig:MotionMixScenario3Sphere}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/CartesianPathDFMain_4.png}
    \caption{Motion Mix - Scenario 4}
    \label{fig:MotionMixScenario4}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/CartesianPathDFMain_5.png}
    \caption{Motion Mix - Scenario 5}
    \label{fig:MotionMixScenario5}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/CartesianPathDFMain_6.png}
    \caption{Motion Mix - Scenario 6}
    \label{fig:MotionMixScenario6}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/CartesianPathDFMain_7.png}
    \caption{Motion Mix - Scenario 7}
    \label{fig:MotionMixScenario7}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/CartesianPathDFMain_PCA3D.png}
    \caption{Evolution and 3D scatter plot of PCA coordinates (x,y,z), calculated in Expanding Window}
    \label{fig:MotionMixScenario7}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/curvature_plot_sphere.png}
    \caption{Curvature plot for a sphere random sample}
    \label{fig:curvature_plot_sphere}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/curvature_plot_torus.png}
    \caption{Curvature plot for a torus random sample}
    \label{fig:curvature_plot_torus}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/curvature_plot_hyperboloid.png}
    \caption{Curvature plot for a hyperboloid random sample}
    \label{fig:curvature_plot_hyperboloid}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/curvature_plot_ExpWindow_PCA_3D.png}
    \caption{Curvature plot for the Expanding Window PCA market dataset}
    \label{fig:curvature_plot_ExpWindow_PCA_3D}
\end{figure}

==> notes.tex <==
We define the marginal risk contribution ($MR_m$), which reflects the effect of a (small) change in the $m-th$ asset's  portfolio weight, with $m=1,2,\dots,D$, on the total portfolio risk. As such, by denoting the total portfolio's variance as $\sigma_p$, the individual asset's portfolio weight as $w_m$, its variance as $\sigma_m$ and its covariance with another asset $l$ in the portfolio as $\sigma_{ml}$ (\citep{Braga2015}), we have : %\textcolor{red}{WE NEED CITATION}

\begin{equation}
{MR}_m = \frac{\partial \sigma_p}{\partial w_m} = \frac{w_m \sigma_m^2 + \sum_{m \neq l}^D w_l \sigma_{ml}}{\sigma_p}.
\end{equation}

\textbf{PANAGIOTI BRHKA AUTO TO PAPER POU EKANES CITE. KATARXAS AUTO KANEI CITE ALLA PAPERS POU PRPEEI NA DEIS KAI NA KANEIS CITE... EPISIS GIA TO SIGMA P TO ORIZEI PROTA PRIN ORISEI TIS EPOMENS SXESEIS KAI DEN TO ORIZEI OS THN SXESH 18! POU EINAI H SXESH 18 SE AYTO TO PAPER?}
We also define the total risk contribution $RC_m$ or otherwise stated as component risk, which reflects the total risk contributed by the position $w_m$ (\citep{Braga2015}), as : %\textcolor{red}{WE NEED CITATION}

\begin{equation}
{RC}_m = w_m \frac{\partial \sigma_p}{\partial w_m} = w_m \frac{w_m \sigma_m^2 + \sum_{m \neq l}^D w_l \sigma_{ml}}{\sigma_p}.
\end{equation}

Following the concepts of capital allocation methodologies, thoroughly researched and documented in several research papers, as in \citep{Koyluoglu2002}, \citep{Urban2003}, and more specifically the context of the so called Euler principle, as defined and investigated in \citep{McNeil2015} and in \citep{Tasche2008}, the application of Euler's theorem for homogeneous functions \citep{Heinrich1994} on portfolio risk analysis, suggests that we consider the total portfolio risk to be a homogeneous function of order 1. Applying the theorem in our context, we get an expression for the total portfolio risk, as the sum of individual risk contributions :
%\textcolor{red}{ANAGIOTI AFOI TO EGRAPSES ETSI PREPEI NA TO APODEIKSEIS KIOLAS, DHLADH NA BALEIS TIS PRAKSEIS} ---- \textcolor{red}{PANAGIOTI THIS CANT BE CORRECT: ABOVE (14) sp appears in the denominator of RC and then BELOW (15) you define this again . If you take the sum this IS NOT SATISFIED}:

\begin{equation}
\sigma_p = \sum_{m=1}^{D} {RC}_m
\end{equation}

The percentage total risk contribution ($PTRC_m$) of each $m$ position is defined as : %\textcolor{red}{WE NEED CITATION}

\begin{equation}
   {PTRC}_m = \frac{w_m \frac{\partial \sigma_p}{\partial w_m}}{\sigma_p}
\end{equation}

As again stated in \citep{Braga2015}, this expression finally provides the target condition for the risk parity strategy, as the equalisation of the total risk contributions $\forall m,l$ :

\begin{equation}
   \frac{w_m \frac{\partial \sigma_p}{\partial w_m}}{\sigma_p} = \frac{w_l \frac{\partial \sigma_p}{\partial w_l}}{\sigma_p}, 
\end{equation}

The portfolio weights are inversely connected to each asset's volatility as well its correlation to the other assets in the portfolio. Since the portfolio weights as defined in this context, and under the constraints $\sum_{m=1}^{D} w_m = 1$ and $0 \leq w_m \leq 1$ the problem of finding the optimal solution for the weights is not feasible, since there is an issue of endogeneity, i.e. the $w_m$ weight is a function of the $RC$s, which again are functions of the weights themselves. A numerical optimization approach was proposed for this problem, by \citep{Maillard2010} and is defined below as :

\begin{equation}
    \min_{w*} = \sum_{m=1}^{D} \sum_{l=1}^{D} ( \frac{w_m \frac{\partial \sigma_p}{\partial w_m}}{\sigma_p} - \frac{w_l \frac{\partial \sigma_p}{\partial w_l}}{\sigma_p} ), \forall m,l 
\end{equation}

from which we can also see that in the case where the assets have the same pair-wise correlations, then the optimal ERC portfolio weights are proportional to the inverse standard deviation or inverse risk. Under this rationale then the optimal weights are computed as :

\begin{equation}
    w_m  = \frac{\frac{1}{\sigma_m}}{\sum_{m=1}^{D} \frac{1}{\sigma_m}}
\end{equation}


///////////////////////////////// 30-7-2021 ///////////////////////////////



\subsection*{2. Covariance Matrix Computation}

For the points in the current window \(\mathcal{W}_t = \{\mathbf{p}_i = (x_i, y_i, z_i) \mid i \in \mathcal{W}_t\}\), compute the covariance matrix:
\[
\mathbf{C}_t = \frac{1}{|\mathcal{W}_t|} \sum_{i \in \mathcal{W}_t} (\mathbf{p}_i - \bar{\mathbf{p}}_t)(\mathbf{p}_i - \bar{\mathbf{p}}_t)^\top,
\]
where:
\begin{itemize}
    \item \(\bar{\mathbf{p}}_t = \frac{1}{|\mathcal{W}_t|} \sum_{i \in \mathcal{W}_t} \mathbf{p}_i\): Mean vector of the points in the window,
    \item \(\mathbf{C}_t \in \mathbb{R}^{3 \times 3}\): Covariance matrix representing the variability of the point cloud.
\end{itemize}

\subsection*{3. Eigenvalue and Eigenvector Decomposition}

The covariance matrix \(\mathbf{C}_t\) is decomposed into eigenvalues and eigenvectors:
\[
\mathbf{C}_t = \mathbf{Q}_t \boldsymbol{\Lambda}_t \mathbf{Q}_t^\top,
\]
where:
\begin{itemize}
    \item \(\boldsymbol{\Lambda}_t = \text{diag}(\lambda_{t,1}, \lambda_{t,2}, \lambda_{t,3})\): Diagonal matrix of eigenvalues sorted as \(\lambda_{t,1} \geq \lambda_{t,2} \geq \lambda_{t,3}\),
    \item \(\mathbf{Q}_t = [\mathbf{q}_{t,1}, \mathbf{q}_{t,2}, \mathbf{q}_{t,3}]\): Matrix of eigenvectors, where each \(\mathbf{q}_{t,i}\) corresponds to eigenvalue \(\lambda_{t,i}\).
\end{itemize}


\subsection*{4. Normalization of Eigenvalues}

To compare the eigenvalues across time, they are normalized:
\[
\tilde{\lambda}_{t,i} = \frac{\lambda_{t,i}}{\sum_{j=1}^3 \lambda_{t,j}}, \quad i \in \{1, 2, 3\}.
\]
The normalized eigenvalues \(\tilde{\lambda}_{t,i}\) sum to 1:
\[
\sum_{i=1}^3 \tilde{\lambda}_{t,i} = 1.
\]

\subsection*{5. Absolute Eigenvector Components}

To analyze the orientation of eigenvectors over time, the absolute values of eigenvector components are computed:
\[
\tilde{\mathbf{q}}_{t,i} = |\mathbf{q}_{t,i}|, \quad i \in \{1, 2, 3\}.
\]





////////////////// SUP MATERIAL 1 /////////////////
We construct seven Brownian motion configurations (motion sequences) on the target underlying geometries : \\ 

\textbf{Scenario 1} : Patterned Sequence

\begin{align*}
&\text{Sphere} \rightarrow \text{Hyperbolic space} \rightarrow \text{Euclidean space} \\
&\rightarrow \text{Sphere} \rightarrow \text{Hyperbolic space} \rightarrow \text{Euclidean space} \\
&\rightarrow \text{Sphere} \rightarrow \text{Hyperbolic space} \rightarrow \text{Euclidean space} \\
&\rightarrow \text{Sphere}
\end{align*}

\textbf{Scenario 2} : Randomized Sequence

\begin{align*}
&\text{Sphere} \rightarrow \text{Hyperbolic space} \rightarrow \text{Euclidean space} \\
&\rightarrow \text{Hyperbolic space} \rightarrow \text{Euclidean space} \rightarrow \text{Hyperbolic space} \\
&\rightarrow \text{Sphere} \rightarrow \text{Euclidean space} \rightarrow \text{Hyperbolic space} \\
&\rightarrow \text{Sphere}
\end{align*}
 
\textbf{Scenario 3} : Single Manifold (Sphere)
 \\
\textbf{Scenario 4} : Single Manifold (Torus)
 \\
\textbf{Scenario 5} : Single Manifold (Euclidean)
 \\
\textbf{Scenario 6} : Repeated Hyperbolic Space
 \\
\textbf{Scenario 7} : Extended Pattern with Torus (6 repeats)
 
\begin{align*}
&\text{Sphere} \rightarrow \text{Hyperbolic space} \rightarrow \text{Euclidean space} \rightarrow \text{Torus} 
\end{align*}


////////////////// SUP MATERIAL 2 /////////////////

The dataset used in this study encompasses a broad spectrum of financial assets, covering the period from January 1, 2005, to August 3, 2025. The assets include:

\begin{itemize}
    \item \textbf{Broad Market Indices}: S\&P 500 (SPY), NASDAQ-100 (QQQ), Dow Jones Industrial Average (DIA), Russell 2000 (IWM), MSCI Emerging Markets (EEM), and MSCI EAFE (EFA).
    \item \textbf{Sector ETFs}: Technology Select Sector SPDR (XLK), Financial Select Sector SPDR (XLF), Health Care Select Sector SPDR (XLV), Energy Select Sector SPDR (XLE), Consumer Discretionary Select Sector SPDR (XLY), Consumer Staples Select Sector SPDR (XLP), Utilities Select Sector SPDR (XLU), Industrial Select Sector SPDR (XLI), and Materials Select Sector SPDR (XLB).
    \item \textbf{Bond ETFs}: iShares 20+ Year Treasury Bond ETF (TLT), iShares 7-10 Year Treasury Bond ETF (IEF), iShares 1-3 Year Treasury Bond ETF (SHY), iShares iBoxx \$ Investment Grade Corporate Bond ETF (LQD), iShares iBoxx \$ High Yield Corporate Bond ETF (HYG), iShares TIPS Bond ETF (TIP), and iShares MBS ETF (MBB).
    \item \textbf{Commodity ETFs}: SPDR Gold Shares (GLD), iShares Silver Trust (SLV), Invesco DB Agriculture Fund (DBA), Teucrium Corn Fund (CORN), Invesco DB Base Metals Fund (DBB), Aberdeen Standard Physical Platinum Shares ETF (PPLT), and Aberdeen Standard Physical Palladium Shares ETF (PALL).
    \item \textbf{Oil ETFs}: United States Oil Fund (USO), ProShares Ultra Bloomberg Crude Oil (UCO), Invesco DB Oil Fund (DBO), and SPDR S\&P Oil \& Gas Exploration \& Production ETF (XOP).
    \item \textbf{Non-U.S. ETFs}: iShares MSCI ACWI ex U.S. ETF (ACWX), Vanguard FTSE All-World ex-US ETF (VEU), iShares MSCI Europe ETF (IEUR), iShares MSCI Pacific ex Japan ETF (EPP), iShares Latin America 40 ETF (ILF), iShares MSCI Canada ETF (EWC), iShares MSCI United Kingdom ETF (EWU), iShares MSCI South Korea ETF (EWY), iShares MSCI Australia ETF (EWA), iShares MSCI Taiwan ETF (EWT), and Vanguard FTSE Emerging Markets ETF (VWO).
    \item \textbf{Dividend and Volatility ETFs}: Vanguard Dividend Appreciation ETF (VIG), iShares Select Dividend ETF (DVY), SPDR S\&P Dividend ETF (SDY), and ProShares VIX Short-Term Futures ETF (VIXY).
    \item \textbf{Alternative ETFs}: iShares Clean Energy ETF (ICLN) and Global X Lithium \& Battery Tech ETF (LIT).
\end{itemize}

This diverse dataset provides comprehensive coverage of global financial markets, enabling robust testing of the proposed methodologies across various asset classes and economic regimes.

------------------------------------------------------------
(KEEP ?)
\textbf{Unbiased estimators}\\

Expanding window analysis aligns closely with the concept of unbiased estimators in statistics, which aim to provide parameter estimates without systematic error (bias). By using an expanding window, we reduce the bias introduced by limited sample sizes and ensure that the estimator asymptotically approaches the true parameter value as the window grows.

Let \(\lambda_i(t)\) denote the eigenvalue of the \(i\)-th principal component at time \(t\), calculated using a covariance matrix \(\mathbf{\Sigma}(t)\) derived from an expanding window of observations \(\{R_{t-\tau}, \dots, R_t\}\), where \(\tau\) increases over time. The unbiasedness of \(\lambda_i(t)\) can be expressed as:

\begin{equation}
\mathbb{E}[\lambda_i(t)] = \lambda_i^*, \quad \forall t,
\end{equation}

where \(\lambda_i^*\) is the true eigenvalue of the population covariance matrix. Expanding windows mitigate bias by leveraging more data points, reducing sampling variability and improving the accuracy of estimates. The mean squared error (MSE) of \(\lambda_i(t)\), combining bias and variance, can be minimized as:

\begin{equation}
\text{MSE}[\lambda_i(t)] = \text{Bias}^2[\lambda_i(t)] + \text{Var}[\lambda_i(t)],
\end{equation}

where the bias decreases with larger sample sizes due to the expanding window. This property is consistent with findings in statistical literature on unbiased estimators.

In financial applications, unbiased eigenvalue estimation is critical for weighting eigenportfolios based on their explanatory power. Using expanding windows ensures that portfolio weights derived from eigenvalues are robust to structural breaks and regime shifts, as demonstrated in prior research on forecasting models. The weights for the \(i\)-th eigenportfolio are dynamically adjusted as:

\begin{equation}
C_{i,t} = \frac{\lambda_i(t)}{\sum_{j=1}^k \lambda_j(t)},
\end{equation}

where \(k\) is the number of principal components retained. This weighting scheme ensures that portfolios with higher eigenvalues—indicating greater variance explained—receive proportionally higher allocations.
